uPredict: A User-Level Profiler-Based Predictive Framework for Single VM Applications in Multi-Tenant Clouds

Most existing studies on performance prediction for virtual machines (VMs) in multi-tenant clouds are at system level and generally require access to performance counters in Hypervisors. In this work, we propose uPredict, a user-level profiler-based performance predictive framework for single-VM applications in multi-tenant clouds. Here, three micro-benchmarks are specially devised to assess the contention of CPUs, memory and disks in a VM, respectively. Based on measured performance of an application and micro-benchmarks, the application and VM-specific predictive models can be derived by exploiting various regression and neural network based techniques. These models can then be used to predict the application's performance using the in-situ profiled resource contention with the micro-benchmarks. We evaluated uPredict extensively with representative benchmarks from PARSEC, NAS Parallel Benchmarks and CloudSuite, on both a private cloud and two public clouds. The results show that the average prediction errors are between 9.8% to 17% for various predictive models on the private cloud with high resource contention, while the errors are within 4% on public clouds. A smart load-balancing scheme powered by uPredict is presented and can effectively reduce the execution and turnaround times of the considered application by 19% and 10%, respectively.

==> 19-sc-bib-new.tex <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{65}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[\protect\citeauthoryear{Abadi, Agarwal, Barham, Brevdo, Chen, Citro,
   Corrado, Davis, Dean, Devin, Ghemawat, Goodfellow, Harp, Irving, Isard, Jia,
   Jozefowicz, Kaiser, Kudlur, Levenberg, Man\'{e}, Monga, Moore, Murray, Olah,
   Schuster, Shlens, Steiner, Sutskever, Talwar, Tucker, Vanhoucke, Vasudevan,
   Vi\'{e}gas, Vinyals, Warden, Wattenberg, Wicke, Yu, and Zheng}{Abadi
   et~al\mbox{.}}{2015}]%
         {tensorflow2015}
 \bibfield{author}{\bibinfo{person}{M. Abadi}, \bibinfo{person}{A.
   Agarwal}, \bibinfo{person}{P. Barham}, \bibinfo{person}{E. Brevdo},
   \bibinfo{person}{Z. Chen}, \bibinfo{person}{C. Citro},
   \bibinfo{person}{G. Corrado}, \bibinfo{person}{A. Davis},
   \bibinfo{person}{J. Dean}, \bibinfo{person}{M. Devin},
   \bibinfo{person}{S. Ghemawat}, \bibinfo{person}{I. Goodfellow},
   \bibinfo{person}{A. Harp}, \bibinfo{person}{G. Irving},
   \bibinfo{person}{M. Isard}, \bibinfo{person}{Y. Jia},
   \bibinfo{person}{R. Jozefowicz}, \bibinfo{person}{L. Kaiser},
   \bibinfo{person}{M. Kudlur}, \bibinfo{person}{J. Levenberg},
   \bibinfo{person}{D. Man\'{e}}, \bibinfo{person}{R. Monga},
   \bibinfo{person}{S. Moore}, \bibinfo{person}{D. Murray},
   \bibinfo{person}{C. Olah}, \bibinfo{person}{M. Schuster},
   \bibinfo{person}{J. Shlens}, \bibinfo{person}{B. Steiner},
   \bibinfo{person}{I. Sutskever}, \bibinfo{person}{K. Talwar},
   \bibinfo{person}{P. Tucker}, \bibinfo{person}{V. Vanhoucke},
   \bibinfo{person}{V. Vasudevan}, \bibinfo{person}{F. Vi\'{e}gas},
   \bibinfo{person}{O. Vinyals}, \bibinfo{person}{P. Warden},
   \bibinfo{person}{M. Wattenberg}, \bibinfo{person}{M. Wicke},
   \bibinfo{person}{Y. Yu}, {and} \bibinfo{person}{X. Zheng}.}
   \bibinfo{year}{2015}\natexlab{}.
 \newblock \bibinfo{title}{{TensorFlow}: Large-Scale Machine Learning on
   Heterogeneous Systems}.
 \newblock
 \newblock
 \urldef\tempurl%
 \url{https://www.tensorflow.org/}
 \showURL{%
 \tempurl}
 \newblock
 \shownote{Software available from tensorflow.org.}


\bibitem[\protect\citeauthoryear{Agarwal, Kandula, Bruno, Wu, Stoica, and
  Zhou}{Agarwal et~al\mbox{.}}{2012}]%
        {2012-Agarwal-NSDI}
\bibfield{author}{\bibinfo{person}{S. Agarwal}, \bibinfo{person}{S.
  Kandula}, \bibinfo{person}{N. Bruno}, \bibinfo{person}{M. Wu},
  \bibinfo{person}{I. Stoica}, {and} \bibinfo{person}{J. Zhou}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{{Reoptimizing Data Parallel Computing}}. In
  \bibinfo{booktitle}{\emph{Proc. of {USENIX} Symp. on Networked Systems Design and
  Implementation (NSDI)}}.
\newblock


\bibitem[\protect\citeauthoryear{Alipourfard, Liu, Chen, Venkataraman, Yu, and
  Zhang}{Alipourfard et~al\mbox{.}}{2017}]%
        {2017-Alipourfard-NSDI}
\bibfield{author}{\bibinfo{person}{O. Alipourfard},
  \bibinfo{person}{H. Liu}, \bibinfo{person}{J. Chen},
  \bibinfo{person}{S. Venkataraman}, \bibinfo{person}{M. Yu}, {and}
  \bibinfo{person}{M. Zhang}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{CherryPick: Adaptively Unearthing the Best Cloud
  Configurations for Big Data Analytics}}. In
  \bibinfo{booktitle}{\emph{Proc. of {USENIX} Symp. on Networked Systems Design and
  Implementation (NSDI)}}.
\newblock


\bibitem[\protect\citeauthoryear{{Amazon Web Services}}{{Amazon Web
  Services}}{ }]%
        {aws-machine}
\bibfield{author}{\bibinfo{person}{{Amazon Web Services}}.} \bibinfo{year}%{ }\natexlab{}.
\newblock \bibinfo{howpublished}{https://aws.amazon.com/ec2/}. last accessed, 2019.
\newblock


\bibitem[\protect\citeauthoryear{Bailey}{Bailey}{2011}]%
        {nas}
\bibfield{author}{\bibinfo{person}{D. Bailey}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Nas parallel benchmarks}.
\newblock In \bibinfo{booktitle}{\emph{Encyclopedia of Parallel Computing}}.
  \bibinfo{publisher}{Springer}, \bibinfo{pages}{1254--1259}.
\newblock


\bibitem[\protect\citeauthoryear{Ballani, Karagiannis, Rowstron, and
  Costa}{Ballani et~al\mbox{.}}{2011}]%
        {2011-Ballani-SIGCOMM}
\bibfield{author}{\bibinfo{person}{H. Ballani}, \bibinfo{person}{T.
  Karagiannis}, \bibinfo{person}{A. Rowstron}, {and} \bibinfo{person}{P.
  Costa}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{Towards Predictable Datacenter Networks}}. In
  \bibinfo{booktitle}{\emph{Proc. of ACM SIGCOMM Conf. on Data Communication
  (SIGCOMM)}}.
\newblock


\bibitem[\protect\citeauthoryear{{Baughman}, {Chard}, {Ward}, {Pitt}, {Chard},
  and {Foster}}{{Baughman} et~al\mbox{.}}{2018}]%
        {2018-Baughman-UCC}
\bibfield{author}{\bibinfo{person}{M. {Baughman}}, \bibinfo{person}{R.
  {Chard}}, \bibinfo{person}{L. {Ward}}, \bibinfo{person}{J. {Pitt}},
  \bibinfo{person}{K. {Chard}}, {and} \bibinfo{person}{I. {Foster}}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{Profiling and Predicting Application Performance
  on the Cloud}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l Conf. on Utility and Cloud
  Computing ({UCC})}}.
\newblock


\bibitem[\protect\citeauthoryear{Begam, Moradi, Wang, and Zhu}{Begam
  et~al\mbox{.}}{2018}]%
        {begam-cloud-2018}
\bibfield{author}{\bibinfo{person}{R. Begam}, \bibinfo{person}{H.
  Moradi}, \bibinfo{person}{W. Wang}, {and} \bibinfo{person}{D. Zhu}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Flexible VM Provisioning for Time-Sensitive
  Applications with Multiple Execution Options}. In
  \bibinfo{booktitle}{\emph{Proc. of IEEE Int'l Conf. on Cloud
  Computing (CLOUD)}}.
\newblock


\bibitem[\protect\citeauthoryear{Bergstra, Bardenet, Bengio, and
  K{\'e}gl}{Bergstra et~al\mbox{.}}{2011}]%
        {2011-Bergstra-NIPS}
\bibfield{author}{\bibinfo{person}{J. Bergstra}, \bibinfo{person}{R.
  Bardenet}, \bibinfo{person}{Y. Bengio}, {and} \bibinfo{person}{B.
  K{\'e}gl}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{Algorithms for Hyper-parameter Optimization}}. In
  \bibinfo{booktitle}{\emph{Proc. of Int'l Conf. on Neural Information
  Processing Systems (NIPS)}}.
\newblock


\bibitem[\protect\citeauthoryear{Bienia}{Bienia}{2011}]%
        {PARSEC}
\bibfield{author}{\bibinfo{person}{C. Bienia}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \emph{\bibinfo{title}{Benchmarking Modern Multiprocessors}}.
\newblock \bibinfo{thesistype}{Ph.D. Dissertation}. \bibinfo{school}{Princeton
  University}.
\newblock


\bibitem[\protect\citeauthoryear{Bishop}{Bishop}{1995}]%
        {1995-Bishop-NeuralBook}
\bibfield{author}{\bibinfo{person}{C. Bishop}.}
  \bibinfo{year}{1995}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{{Neural networks for pattern
  recognition}}}.
\newblock \bibinfo{publisher}{Oxford university press}.
\newblock


\bibitem[\protect\citeauthoryear{{Clemente-Castelló}, {Nicolae}, {Mayo}, and
  {Fernández}}{{Clemente-Castelló} et~al\mbox{.}}{2018}]%
        {2018-CLemente-TPDS}
\bibfield{author}{\bibinfo{person}{F.~J. {Clemente-Castello}},
  \bibinfo{person}{B. {Nicolae}}, \bibinfo{person}{R. {Mayo}}, {and}
  \bibinfo{person}{J.~C. {Fernandez}}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{Performance Model of MapReduce Iterative
  Applications for Hybrid Cloud Bursting}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Parallel and Distributed
  Systems}} \bibinfo{volume}{29}, \bibinfo{number}{8} (\bibinfo{year}{2018}),
  \bibinfo{pages}{1794--1807}.
\newblock


\bibitem[\protect\citeauthoryear{Dejun, Pierre, and Chi}{Dejun
  et~al\mbox{.}}{2011}]%
        {2011-Jiang-Webapps}
\bibfield{author}{\bibinfo{person}{J. Dejun}, \bibinfo{person}{G.
  Pierre}, {and} \bibinfo{person}{C. Chi}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Resource provisioning of web applications in
  heterogeneous clouds}. In \bibinfo{booktitle}{\emph{Proc. of USENIX conf. on Web Application Development ({WebApps})}}.
\newblock


\bibitem[\protect\citeauthoryear{Delimitrou and Kozyrakis}{Delimitrou and
  Kozyrakis}{2013a}]%
        {ibench}
\bibfield{author}{\bibinfo{person}{C. Delimitrou} {and} \bibinfo{person}{C.
  Kozyrakis}.} \bibinfo{year}{2013}\natexlab{a}.
\newblock \showarticletitle{{iBench: Quantifying interference for datacenter
  applications}}. In \bibinfo{booktitle}{\emph{Proc. of IEEE Int'l Symp. on
  Workload Characterization (IISWC)}}.
\newblock


\bibitem[\protect\citeauthoryear{Delimitrou and Kozyrakis}{Delimitrou and
  Kozyrakis}{2013b}]%
        {christina}
\bibfield{author}{\bibinfo{person}{C. Delimitrou} {and}
  \bibinfo{person}{C. Kozyrakis}.} \bibinfo{year}{2013}\natexlab{b}.
\newblock \showarticletitle{{Paragon: QoS-aware Scheduling for Heterogeneous
  Datacenters}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l
  Conf. on Architectural Support for Programming Languages and Operating
  Systems (ASPLOS)}}.
\newblock


\bibitem[\protect\citeauthoryear{Delimitrou and Kozyrakis}{Delimitrou and
  Kozyrakis}{2014}]%
        {2014-Delimitrou-ASPLOS}
\bibfield{author}{\bibinfo{person}{C. Delimitrou} {and}
  \bibinfo{person}{C. Kozyrakis}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{{Quasar: Resource-efficient and QoS-aware Cluster
  Management}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l Conf. on
  Architectural Support for Programming Languages and Operating Systems (ASPLOS)}}.
\newblock


\bibitem[\protect\citeauthoryear{Farley, Juels, Varadarajan, Ristenpart,
  Bowers, and Swift}{Farley et~al\mbox{.}}{2012}]%
        {2012-Farley-SoCC}
\bibfield{author}{\bibinfo{person}{B. Farley}, \bibinfo{person}{A.
  Juels}, \bibinfo{person}{V. Varadarajan}, \bibinfo{person}{T.
  Ristenpart}, \bibinfo{person}{K.~D. Bowers}, {and}
  \bibinfo{person}{M.~M. Swift}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{More for Your Money: Exploiting Performance
  Heterogeneity in Public Clouds}. In \bibinfo{booktitle}{\emph{Proc. of
 ACM Symp. on Cloud Computing ({SoCC})}}.
\newblock


\bibitem[\protect\citeauthoryear{Ferdman, Adileh, Kocberber, Volos, Alisafaee,
  Jevdjic, Kaynak, Popescu, Ailamaki, and Falsafi}{Ferdman
  et~al\mbox{.}}{2012}]%
        {cloudsuit}
\bibfield{author}{\bibinfo{person}{M. Ferdman}, \bibinfo{person}{A.
  Adileh}, \bibinfo{person}{O. Kocberber}, \bibinfo{person}{S. Volos},
  \bibinfo{person}{M. Alisafaee}, \bibinfo{person}{D. Jevdjic},
  \bibinfo{person}{C. Kaynak}, \bibinfo{person}{A.~D. Popescu},
  \bibinfo{person}{A. Ailamaki}, {and} \bibinfo{person}{B. Falsafi}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Clearing the Clouds: A Study of Emerging Scale-out
  Workloads on Modern Hardware}. In
\newblock \bibinfo{journal}{\emph{Proc. of Int'l Conf. on Architectural Support for Programming Languages and Operating
  Systems (ASPLOS)}}.
\newblock


\bibitem[\protect\citeauthoryear{Ferguson, Bodik, Kandula, Boutin, and
  Fonseca}{Ferguson et~al\mbox{.}}{2012}]%
        {2012-Ferguson-EuroSys}
\bibfield{author}{\bibinfo{person}{A.~D. Ferguson}, \bibinfo{person}{P.
  Bodik}, \bibinfo{person}{S. Kandula}, \bibinfo{person}{E. Boutin},
  {and} \bibinfo{person}{R. Fonseca}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{{Jockey: Guaranteed Job Latency in Data Parallel
  Clusters}}. In \bibinfo{booktitle}{\emph{Proc. of ACM European Conf. on
  Computer Systems ({EuroSys})}}.
\newblock


\bibitem[\protect\citeauthoryear{{Friese}, {Tallent}, {Vishnu}, {Kerbyson}, and
  {Hoisie}}{{Friese} et~al\mbox{.}}{2017}]%
        {2017-Friese-IPDPS}
\bibfield{author}{\bibinfo{person}{R.~D. {Friese}}, \bibinfo{person}{N.~R.
  {Tallent}}, \bibinfo{person}{A. {Vishnu}}, \bibinfo{person}{D.~J.
  {Kerbyson}}, {and} \bibinfo{person}{A. {Hoisie}}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Generating Performance Models for Irregular
  Applications}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l Parallel and Distributed
  Processing Symp. ({IPDPS})}}.
\newblock


\bibitem[\protect\citeauthoryear{{Google Compute Engine}}{{Google Compute
  Engine}}{ }]%
        {google-machine}
\bibfield{author}{\bibinfo{person}{{Google Compute Engine}}.}
  \bibinfo{year}%{ }\natexlab{}.
\newblock \bibinfo{howpublished}{https://cloud.google.com/}. last accessed, 2019.
\newblock


\bibitem[\protect\citeauthoryear{Govindan, Liu, Kansal, and
  Sivasubramaniam}{Govindan et~al\mbox{.}}{2011}]%
        {cuanta2011}
\bibfield{author}{\bibinfo{person}{S. Govindan}, \bibinfo{person}{J. Liu},
  \bibinfo{person}{A. Kansal}, {and} \bibinfo{person}{A.
  Sivasubramaniam}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{Cuanta: Quantifying Effects of Shared On-chip
  Resource Interference for Consolidated Virtual Machines}}. In
  \bibinfo{booktitle}{\emph{Proc. of ACM Symp. on Cloud Computing ({SoCC})}}.
\newblock


\bibitem[\protect\citeauthoryear{Gunn et~al\mbox{.}}{Gunn
  et~al\mbox{.}}{1998b}]%
        {1998-Gunn-ISISTR}
\bibfield{author}{\bibinfo{person}{S.~R. Gunn}}
  \bibinfo{year}{1998}\natexlab{b}.
\newblock \showarticletitle{Support vector machines for classification and
  regression}.
\newblock \bibinfo{journal}{\emph{University of Southampton technical report}}
  \bibinfo{volume}{14}, \bibinfo{number}{1} (\bibinfo{year}{1998}),
  \bibinfo{pages}{5--16}.
\newblock


\bibitem[\protect\citeauthoryear{Hecht-Nielsen}{Hecht-Nielsen}{1992}]%
        {neuralnetwork1992}
\bibfield{author}{\bibinfo{person}{R. Hecht-Nielsen}.}
  \bibinfo{year}{1992}\natexlab{}.
\newblock \showarticletitle{Theory of the backpropagation neural network}.
\newblock In \bibinfo{booktitle}{\emph{Neural Networks for Perception}}.
  \bibinfo{publisher}{Elsevier}, \bibinfo{pages}{65--93}.
\newblock


\bibitem[\protect\citeauthoryear{Hoerl and Kennard}{Hoerl and Kennard}{1970}]%
        {hoerl1970ridge}
\bibfield{author}{\bibinfo{person}{A.~E. Hoerl} {and}
  \bibinfo{person}{R.~W. Kennard}.} \bibinfo{year}{1970}\natexlab{}.
\newblock \showarticletitle{{Ridge regression: applications to nonorthogonal
  problems}}.
\newblock \bibinfo{journal}{\emph{Technometrics}} \bibinfo{volume}{12},
  \bibinfo{number}{1} (\bibinfo{year}{1970}), \bibinfo{pages}{69--82}.
\newblock


\bibitem[\protect\citeauthoryear{Hornik, Stinchcombe, and White}{Hornik
  et~al\mbox{.}}{1989}]%
        {1989-HORNIK-NN}
\bibfield{author}{\bibinfo{person}{K. Hornik}, \bibinfo{person}{Maxwell
  Stinchcombe}, {and} \bibinfo{person}{Halbert White}.}
  \bibinfo{year}{1989}\natexlab{}.
\newblock \showarticletitle{{Multilayer Feedforward Networks are Universal
  Approximators}}.
\newblock \bibinfo{journal}{\emph{Neural Networks}} \bibinfo{volume}{2},
  \bibinfo{number}{5} (\bibinfo{year}{1989}), \bibinfo{pages}{359 -- 366}.
\newblock


\bibitem[\protect\citeauthoryear{Hwang, Bai, Shi, Li, Chen, and Wu}{Hwang
  et~al\mbox{.}}{2016}]%
        {19d}
\bibfield{author}{\bibinfo{person}{K. Hwang}, \bibinfo{person}{X. Bai},
  \bibinfo{person}{Y. Shi}, \bibinfo{person}{M. Li}, \bibinfo{person}{W. Chen},
  {and} \bibinfo{person}{Y. Wu}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{Cloud Performance Modeling with Benchmark
  Evaluation of Elastic Scaling Strategies}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Parallel and Distributed
  Systems}} \bibinfo{volume}{27} \bibinfo{number}{1} (\bibinfo{year}{2016}),
  \bibinfo{pages}{130--143}.
\newblock


\bibitem[\protect\citeauthoryear{{HyperOpt}}{{HyperOpt}}{ }]%
        {hyperopt}
\bibfield{author}{\bibinfo{person}{{HyperOpt}}.} \bibinfo{year}%{ }\natexlab{}.
\newblock \bibinfo{howpublished}{https://github.com/hyperopt/hyperopt}. last accessed, 2019.
\newblock


\bibitem[\protect\citeauthoryear{Iosup, Ostermann, Yigitbasi, Prodan,
  Fahringer, and Epema}{Iosup et~al\mbox{.}}{2011}]%
        {2011-Iosup-TPDS}
\bibfield{author}{\bibinfo{person}{A. Iosup}, \bibinfo{person}{S. Ostermann},
  \bibinfo{person}{M.~N. Yigitbasi}, \bibinfo{person}{R. Prodan},
  \bibinfo{person}{T. Fahringer}, {and} \bibinfo{person}{D. Epema}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{Performance Analysis of Cloud Computing Services
  for Many-Tasks Scientific Computing}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Parallel and Distributed
  Systems}} \bibinfo{volume}{22} \bibinfo{number}{6} (\bibinfo{year}{2011}),
  \bibinfo{pages}{931--945}.
\newblock


\bibitem[\protect\citeauthoryear{{Iosup}, {Yigitbasi}, and {Epema}}{{Iosup}
  et~al\mbox{.}}{2011}]%
        {2011-Iosup-CCGrid}
\bibfield{author}{\bibinfo{person}{A. {Iosup}}, \bibinfo{person}{N.
  {Yigitbasi}}, {and} \bibinfo{person}{D. {Epema}}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{On the Performance Variability of Production Cloud
  Services}}. In \bibinfo{booktitle}{\emph{Proc. of IEEE/ACM Int'l
  Symp. on Cluster, Cloud and Grid Computing ({CCGrid})}}.
\newblock


\bibitem[\protect\citeauthoryear{Leitner and Cito}{Leitner and Cito}{2016}]%
        {2016-Leitner-TOIT}
\bibfield{author}{\bibinfo{person}{P. Leitner} {and}
  \bibinfo{person}{J. Cito}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{Patterns in the Chaos - A Study of
  Performance Variation and Predictability in Public IaaS Clouds}}.
\newblock \bibinfo{journal}{\emph{ACM Transactions on Internet Technology
  (TOIT)}} \bibinfo{volume}{16}, \bibinfo{number}{3} (\bibinfo{year}{2016}),
  \bibinfo{pages}{15:1--15:23}.
\newblock


\bibitem[\protect\citeauthoryear{Li, Wu, Chen, Wang, and Huang}{Li
  et~al\mbox{.}}{2017}]%
        {NICBLE2017}
\bibfield{author}{\bibinfo{person}{H. Li}, \bibinfo{person}{Y. Wu},
  \bibinfo{person}{Y. Chen}, \bibinfo{person}{C. Wang}, {and}
  \bibinfo{person}{Y. Huang}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Application Execution Time Prediction for
  Effective CPU Provisioning in Virtualization Environment}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Parallel and Distributed
  Systems}} \bibinfo{volume}{28},\bibinfo{number}{11} (\bibinfo{year}{2017}),
  \bibinfo{pages}{3074--3088}.
\newblock


\bibitem[\protect\citeauthoryear{Malawski, Juve, Deelman, and
  Nabrzyski}{Malawski et~al\mbox{.}}{2012}]%
        {2012-Malawski-SC}
\bibfield{author}{\bibinfo{person}{M. Malawski}, \bibinfo{person}{G.
  Juve}, \bibinfo{person}{E. Deelman}, {and} \bibinfo{person}{J.
  Nabrzyski}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{{Cost- and Deadline-constrained Provisioning for
  Scientific Workflow Ensembles in IaaS Clouds}}. In
  \bibinfo{booktitle}{\emph{Proc. of Int'l Conf. on High
  Performance Computing, Networking, Storage and Analysis ({SC})}}.
\newblock


\bibitem[\protect\citeauthoryear{Mao and Humphrey}{Mao and Humphrey}{2011}]%
        {2011-SC-Mao}
\bibfield{author}{\bibinfo{person}{M. Mao} {and} \bibinfo{person}{M.
  Humphrey}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{Auto-scaling to Minimize Cost and Meet Application
  Deadlines in Cloud Workflows}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l
  Conf. for High Performance Computing, Networking, Storage and Analysis ({SC})}}.
\newblock


\bibitem[\protect\citeauthoryear{{Mariani}, {Anghel}, {Jongerius}, and
  {Dittmann}}{{Mariani} et~al\mbox{.}}{2017}]%
        {2017-Mariani-CCGRID}
\bibfield{author}{\bibinfo{person}{G. {Mariani}}, \bibinfo{person}{A.
  {Anghel}}, \bibinfo{person}{R. {Jongerius}}, {and} \bibinfo{person}{G.
  {Dittmann}}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Predicting Cloud Performance for HPC Applications:
  A User-Oriented Approach}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l Symp. on
  Cluster, Cloud and Grid Computing ({CCGrid})}}.
\newblock


\bibitem[\protect\citeauthoryear{Maricq, Duplyakin, Jimenez, Maltzahn,
  Stutsman, and Ricci}{Maricq et~al\mbox{.}}{2018}]%
        {2018-Maricq-OSDE}
\bibfield{author}{\bibinfo{person}{A. Maricq}, \bibinfo{person}{D.
  Duplyakin}, \bibinfo{person}{I. Jimenez}, \bibinfo{person}{C. Maltzahn},
  \bibinfo{person}{R. Stutsman}, {and} \bibinfo{person}{R. Ricci}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Taming Performance Variability}. In
  \bibinfo{booktitle}{\emph{Proc. of {USENIX} Symp. on Operating Systems Design
  and Implementation ({OSDI})}}.
\newblock


\bibitem[\protect\citeauthoryear{Mars, Tang, Hundt, Skadron, and Soffa}{Mars
  et~al\mbox{.}}{2011}]%
        {bubbleUp2011}
\bibfield{author}{\bibinfo{person}{J. Mars}, \bibinfo{person}{L. Tang},
  \bibinfo{person}{R. Hundt}, \bibinfo{person}{K. Skadron}, {and}
  \bibinfo{person}{M.~L. Soffa}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{{Bubble-Up: Increasing Utilization in Modern
  Warehouse Scale Computers via Sensible Co-locations}}. In
  \bibinfo{booktitle}{\emph{Proc. of Annual IEEE/ACM Int'l
  Symp. on Microarchitecture ({Micro})}}.
\newblock


\bibitem[\protect\citeauthoryear{Mishra, Lafferty, and Hoffmann}{Mishra
  et~al\mbox{.}}{2017}]%
        {esp2017}
\bibfield{author}{\bibinfo{person}{N. Mishra}, \bibinfo{person}{J.~D.
  Lafferty}, {and} \bibinfo{person}{H. Hoffmann}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{ESP: A Machine Learning Approach to Predicting
  Application Interference}}. In \bibinfo{booktitle}{\emph{Proc. of IEEE Int'l
  Conf. on Autonomic Computing (ICAC)}}.
\newblock


\bibitem[\protect\citeauthoryear{Nathuji, Kansal, and Ghaffarkhah}{Nathuji
  et~al\mbox{.}}{2010}]%
        {qcloud2010eurosys}
\bibfield{author}{\bibinfo{person}{R. Nathuji}, \bibinfo{person}{A.
  Kansal}, {and} \bibinfo{person}{A. Ghaffarkhah}.}
  \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{{Q-clouds: Managing Performance Interference
  Effects for QoS-aware Clouds}}. In \bibinfo{booktitle}{\emph{Proc. of
  ACM European Conf. on Computer Systems ({EuroSys})}}.
\newblock


\bibitem[\protect\citeauthoryear{Novakovi{\'c}, Vasi{\'c}, Novakovi{\'c},
  Kosti{\'c}, and Bianchini}{Novakovi{\'c} et~al\mbox{.}}{2013}]%
        {deepdive2013atc}
\bibfield{author}{\bibinfo{person}{D. Novakovi{\'c}},
  \bibinfo{person}{N. Vasi{\'c}}, \bibinfo{person}{S. Novakovi{\'c}},
  \bibinfo{person}{D. Kosti{\'c}}, {and} \bibinfo{person}{R.
  Bianchini}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{{DeepDive: Transparently Identifying and Managing
  Performance Interference in Virtualized Environments}}. In
  \bibinfo{booktitle}{\emph{Proc. of {USENIX} Annual Technical Conf. ({ATC})}}.
\newblock


\bibitem[\protect\citeauthoryear{Ostermann, Iosup, Yigitbasi, Prodan,
  Fahringer, and Epema}{Ostermann et~al\mbox{.}}{2010}]%
        {2010-Ostermann-CC}
\bibfield{author}{\bibinfo{person}{S. Ostermann},
  \bibinfo{person}{A. Iosup}, \bibinfo{person}{N. Yigitbasi},
  \bibinfo{person}{R. Prodan}, \bibinfo{person}{T. Fahringer}, {and}
  \bibinfo{person}{D. Epema}.} \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{{A Performance Analysis of EC2 Cloud Computing
  Services for Scientific Computing}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l Conf. on Cloud Computing ({CloudComp})}}.
\newblock


\bibitem[\protect\citeauthoryear{Ou, Zhuang, Lukyanenko, Nurminen, Hui,
  Mazalov, and Ylä-Jääski}{Ou et~al\mbox{.}}{2013}]%
        {7est}
\bibfield{author}{\bibinfo{person}{Z. Ou}, \bibinfo{person}{H. Zhuang},
  \bibinfo{person}{A. Lukyanenko}, \bibinfo{person}{J.~K. Nurminen},
  \bibinfo{person}{P. Hui}, \bibinfo{person}{V. Mazalov}, {and}
  \bibinfo{person}{A. Yl{\"a}-J{\"a}{\"a}ski}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{{Is the Same Instance Type Created Equal?
  Exploiting Heterogeneity of Public Clouds}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Cloud Computing}}
  \bibinfo{volume}{1}, \bibinfo{number}{2} (\bibinfo{year}{2013}), \bibinfo{pages}{201--214}.
\newblock


\bibitem[\protect\citeauthoryear{RightScale}{RightScale}{2018}]%
        {2018-RightScale}
\bibfield{author}{\bibinfo{person}{RightScale}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \bibinfo{title}{{State of the Cloud Report}}.
\newblock
\newblock


\bibitem[\protect\citeauthoryear{Romero and Delimitrou}{Romero and
  Delimitrou}{2018}]%
        {Mage2018}
\bibfield{author}{\bibinfo{person}{F. Romero} {and}
  \bibinfo{person}{C. Delimitrou}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{Mage: Online and Interference-Aware Scheduling for
  Multi-Scale Heterogeneous Systems}}. In \bibinfo{booktitle}{\emph{Proc.
  of Int'l Conf. on Parallel Architectures and Compilation
  Techniques (PACT)}}.
\newblock


\bibitem[\protect\citeauthoryear{Rudd, Jain, Scheirer, and Boult}{Rudd
  et~al\mbox{.}}{2018}]%
        {2018-Rudd-TPAMI}
\bibfield{author}{\bibinfo{person}{E.~M. Rudd}, \bibinfo{person}{L.~P.
  Jain}, \bibinfo{person}{W.~J. Scheirer}, {and} \bibinfo{person}{T.~E.
  Boult}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{The Extreme Value Machine}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Pattern Analysis and
  Machine Intelligence}} \bibinfo{volume}{40}, \bibinfo{number}{3}
  (\bibinfo{year}{2018}), \bibinfo{pages}{762--768}.
\newblock


\bibitem[\protect\citeauthoryear{Sarle}{Sarle}{ }]%
        {NNFAQ}
\bibfield{author}{\bibinfo{person}{W.~S. Sarle}.}
\newblock \bibinfo{title}{Neural Network FAQ}.
\newblock \bibinfo{howpublished}{ftp://ftp.sas.com/pub/neural/FAQ.html}. last accessed, 2019.
\newblock


\bibitem[\protect\citeauthoryear{Schad, Dittrich, and Quian{\'e}-Ruiz}{Schad
  et~al\mbox{.}}{2010}]%
        {12d}
\bibfield{author}{\bibinfo{person}{J. Schad}, \bibinfo{person}{J.
  Dittrich}, {and} \bibinfo{person}{J. Quian{\'e}-Ruiz}.}
  \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{{Runtime Measurements in the Cloud: Observing,
  Analyzing, and Reducing Variance}}. In
\newblock \bibinfo{journal}{\emph{Proc. of VLDB Endowment}}.
\newblock


\bibitem[\protect\citeauthoryear{Scheuner and Leitner}{Scheuner and
  Leitner}{2018}]%
        {cloud18}
\bibfield{author}{\bibinfo{person}{J. Scheuner} {and} \bibinfo{person}{P.
  Leitner}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{Estimating Cloud Application Performance Based on
  Micro-Benchmark Profiling}}. In \bibinfo{booktitle}{\emph{Proc. of IEEE Int'l
  Conf. on Cloud Computing ({CLOUD})}}.
\newblock


\bibitem[\protect\citeauthoryear{{Scikit-learn}}{{Scikit-learn}}{ }]%
        {scikit}
\bibfield{author}{\bibinfo{person}{{Scikit-learn}}.} \bibinfo{year}
%{ }\natexlab{}.
\newblock \bibinfo{howpublished}{http://scikit-learn.org/stable/}. last accessed, 2019.
\newblock


\bibitem[\protect\citeauthoryear{{Scikit-Optimize}}{{Scikit-Optimize}}{ }]%
        {scikitoptimize}
\bibfield{author}{\bibinfo{person}{{Scikit-Optimize}}.} \bibinfo{year}%{ }\natexlab{}.
\newblock \bibinfo{howpublished}{https://github.com/scikit-optimize}. last accessed, 2019.
\newblock


\bibitem[\protect\citeauthoryear{Smola and Sch{\"o}lkopf}{Smola and
  Sch{\"o}lkopf}{1998}]%
        {1998-Smola-Algorithmica}
\bibfield{author}{\bibinfo{person}{A.~J. Smola} {and} \bibinfo{person}{B.
  Sch{\"o}lkopf}.} \bibinfo{year}{1998}\natexlab{}.
\newblock \showarticletitle{{On a Kernel-Based Method for Pattern Recognition,
  Regression, Approximation, and Operator Inversion}}.
\newblock \bibinfo{journal}{\emph{Algorithmica}} \bibinfo{volume}{22},
  \bibinfo{number}{1} (\bibinfo{year}{1998}),
  \bibinfo{pages}{211--231}.
\newblock


\bibitem[\protect\citeauthoryear{Snoek, Larochelle, and Adams}{Snoek
  et~al\mbox{.}}{2012}]%
        {2012-Snoek-NIPS}
\bibfield{author}{\bibinfo{person}{J. Snoek}, \bibinfo{person}{H.
  Larochelle}, {and} \bibinfo{person}{R.~P. Adams}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{{Practical Bayesian Optimization of Machine
  Learning Algorithms}}.
\newblock In \bibinfo{booktitle}{\emph{Proc. of Advances in Neural Information
  Processing Systems ({NIPS})}}.
\newblock


\bibitem[\protect\citeauthoryear{{Sontag}}{{Sontag}}{1992}]%
        {1992-Sontag-TNN}
\bibfield{author}{\bibinfo{person}{E.~D. {Sontag}}.}
  \bibinfo{year}{1992}\natexlab{}.
\newblock \showarticletitle{{Feedback Stabilization using Two-hidden-layer
  Nets}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Neural Networks}}
  \bibinfo{volume}{3}, \bibinfo{number}{6} (\bibinfo{date}{Nov}
  \bibinfo{year}{1992}), \bibinfo{pages}{981--990}.
\newblock


\bibitem[\protect\citeauthoryear{{Specht}}{{Specht}}{1991}]%
        {1991-Specht-TNN}
\bibfield{author}{\bibinfo{person}{D.~F. {Specht}}.}
  \bibinfo{year}{1991}\natexlab{}.
\newblock \showarticletitle{{A General Regression Neural Network}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Neural Networks}}
  \bibinfo{volume}{2}, \bibinfo{number}{6} (\bibinfo{year}{1991}),
  \bibinfo{pages}{568--576}.
\newblock


\bibitem[\protect\citeauthoryear{Tang, Mars, Wang, Dey, and Soffa}{Tang
  et~al\mbox{.}}{2013}]%
        {2013-Tang-ASPLOS}
\bibfield{author}{\bibinfo{person}{L. Tang}, \bibinfo{person}{J. Mars},
  \bibinfo{person}{W. Wang}, \bibinfo{person}{T. Dey}, {and}
  \bibinfo{person}{M. Soffa}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{{ReQoS: Reactive Static/Dynamic Compilation for QoS
  in Warehouse Scale Computers}}. In \bibinfo{booktitle}{\emph{Proc. of
  Int'l Conf. on Architectural Support for Programming Languages
  and Operating Systems (ASPLOS)}}.
\newblock


\bibitem[\protect\citeauthoryear{Tibshirani}{Tibshirani}{1996}]%
        {tibshirani1996regression}
\bibfield{author}{\bibinfo{person}{R. Tibshirani}.}
  \bibinfo{year}{1996}\natexlab{}.
\newblock \showarticletitle{{Regression shrinkage and selection via the
  lasso}}.
\newblock \bibinfo{journal}{\emph{Journal of the Royal Statistical Society}} \bibinfo{volume}{58}, \bibinfo{number}{1} (\bibinfo{year}{1996}),
  \bibinfo{pages}{267--288}.
\newblock


\bibitem[\protect\citeauthoryear{Venkataraman, Yang, Franklin, Recht, and
  Stoica}{Venkataraman et~al\mbox{.}}{2016}]%
        {ernest2016nsdi}
\bibfield{author}{\bibinfo{person}{S. Venkataraman},
  \bibinfo{person}{Z. Yang}, \bibinfo{person}{M. Franklin},
  \bibinfo{person}{B. Recht}, {and} \bibinfo{person}{I. Stoica}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{Ernest: Efficient Performance Prediction for
  Large-Scale Advanced Analytics}}. In \bibinfo{booktitle}{\emph{ Proc. of {USENIX}
  Symp. on Networked Systems Design and Implementation ({NSDI})}}.
\newblock


\bibitem[\protect\citeauthoryear{Wolf, Bischof, Calotoiu, Hoefler, Iwainsky,
  Kwasniewski, Mohr, Shudler, Strube, Vogel, and Wittum}{Wolf
  et~al\mbox{.}}{2016}]%
        {2016-Wolf-SPPEXA}
\bibfield{author}{\bibinfo{person}{F. Wolf}, \bibinfo{person}{C.
  Bischof}, \bibinfo{person}{A. Calotoiu}, \bibinfo{person}{T.
  Hoefler}, \bibinfo{person}{C. Iwainsky}, \bibinfo{person}{G.
  Kwasniewski}, \bibinfo{person}{B. Mohr}, \bibinfo{person}{S. Shudler},
  \bibinfo{person}{A. Strube}, \bibinfo{person}{A. Vogel}, {and}
  \bibinfo{person}{G. Wittum}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{Automatic Performance Modeling of HPC
  Applications}}. In \bibinfo{booktitle}{\emph{Software for Exascale Computing}}.  \bibinfo{publisher}{Springer}, \bibinfo{pages}{445--465}.
\newblock


\bibitem[\protect\citeauthoryear{Wyatt, Herbein, Gamblin, Moody, Ahn, and
  Taufer}{Wyatt et~al\mbox{.}}{2018}]%
        {2018-Wyatt-ICPP}
\bibfield{author}{\bibinfo{person}{M.~R. Wyatt},
  \bibinfo{person}{S. Herbein}, \bibinfo{person}{T. Gamblin},
  \bibinfo{person}{A. Moody}, \bibinfo{person}{D.~H. Ahn}, {and}
  \bibinfo{person}{M. Taufer}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{{PRIONN: Predicting Runtime and IO Using Neural
  Networks}}. In \bibinfo{booktitle}{\emph{Proc. of Int'l Conf. on Parallel
  Processing ({ICPP)}}}.
\newblock


\bibitem[\protect\citeauthoryear{Yadwadkar, Hariharan, Gonzalez, Smith, and
  Katz}{Yadwadkar et~al\mbox{.}}{2017}]%
        {paris}
\bibfield{author}{\bibinfo{person}{N.~J. Yadwadkar},
  \bibinfo{person}{B. Hariharan}, \bibinfo{person}{J.~E. Gonzalez},
  \bibinfo{person}{B. Smith}, {and} \bibinfo{person}{R.~H. Katz}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{{Selecting the Best VM Across Multiple Public
  Clouds: A Data-driven Performance Modeling Approach}}. In
  \bibinfo{booktitle}{\emph{Proc. of ACM Symp. on Cloud Computing
  (SoCC)}}.
\newblock


\bibitem[\protect\citeauthoryear{Yang, Breslow, Mars, and Tang}{Yang
  et~al\mbox{.}}{2013}]%
        {2013-Yang-ISCA}
\bibfield{author}{\bibinfo{person}{H. Yang}, \bibinfo{person}{A.
  Breslow}, \bibinfo{person}{J. Mars}, {and} \bibinfo{person}{L.
  Tang}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{{Bubble-flux: Precise Online QoS Management for
  Increased Utilization in Warehouse Scale Computers}}. In
  \bibinfo{booktitle}{\emph{Proc. of Int'l Symp. on Computer Architecture ({ISCA})}}.
\newblock


\bibitem[\protect\citeauthoryear{Zhai, Chen, Zheng, and Li}{Zhai
  et~al\mbox{.}}{2016}]%
        {2016-Zhai-IEEEComputer}
\bibfield{author}{\bibinfo{person}{J. Zhai}, \bibinfo{person}{W. Chen},
  \bibinfo{person}{W. Zheng}, {and} \bibinfo{person}{K. Li}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{{Performance Prediction for Large-Scale Parallel
  Applications Using Representative Replay}}.
\newblock \bibinfo{journal}{\emph{IEEE Transactions on Computers}}  \bibinfo{volume}{65}, \bibinfo{number}{7} (\bibinfo{year}{2016}),
  \bibinfo{pages}{2184--2198}.
\newblock


\bibitem[\protect\citeauthoryear{Zhang, Patuwo, and Hu}{Zhang
  et~al\mbox{.}}{2001}]%
        {NeuralNonlinear}
\bibfield{author}{\bibinfo{person}{G.~P. Zhang}, \bibinfo{person}{B.~E.
  Patuwo}, {and} \bibinfo{person}{M.~Y. Hu}.}
  \bibinfo{year}{2001}\natexlab{}.
\newblock \showarticletitle{{A Simulation Study of Artificial Neural Networks
  for Nonlinear Time-series Forecasting}}.
\newblock \bibinfo{journal}{\emph{Computers \& Operations Research}}
  \bibinfo{volume}{28}, \bibinfo{number}{4} (\bibinfo{year}{2001}),
  \bibinfo{pages}{381--396}.
\newblock


\bibitem[\protect\citeauthoryear{Zhang}{Zhang}{2004}]%
        {sgd2004}
\bibfield{author}{\bibinfo{person}{T. Zhang}.}
  \bibinfo{year}{2004}\natexlab{}.
\newblock \showarticletitle{{Solving Large Scale Linear Prediction Problems
  Using Stochastic Gradient Descent Algorithms}}. In
  \bibinfo{booktitle}{\emph{Proc. of Int'l Conf. on Machine
  Learning ({ICML})}}.
\newblock


\bibitem[\protect\citeauthoryear{Zou and Hastie}{Zou and Hastie}{2005}]%
        {zou2005regularization}
\bibfield{author}{\bibinfo{person}{H. Zou} {and} \bibinfo{person}{T.
  Hastie}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{{Regularization and variable selection via the
  elastic net}}.
\newblock \bibinfo{journal}{\emph{Journal of the Royal Statistical Society}} \bibinfo{volume}{67},
  \bibinfo{number}{2} (\bibinfo{year}{2005}), \bibinfo{pages}{301--320}.
\newblock

\end{thebibliography}


==> SecConclusions.tex <==
Although cloud computing offers great value with its pay-as-you-go pricing model and elasticity, it is still very challenging to fully realize the cost benefits of cloud computing due to the random performance fluctuations experienced by the cloud applications. Without accurate knowledge of the performance, it is very difficult for cloud users to plan their resource allocations on the clouds. However, as ordinary cloud users have limited control and access to the underlying execution environments, they cannot utilize techniques presented by previous studies to predict application performance under contention.
%These fluctuations are mostly caused by the hardware resources among the VMs/applications of multiple cloud tenants. Although there have been studies that investigated predicting application performance under resource contention, few techniques have been proposed to address this prediction problem from the perspective of ordinary cloud user 
In this paper, we explored the performance prediction methodology from an ordinary user's perspective. The proposed methodology employs micro-benchmarks and regression / Machine Learning techniques to estimate the severity of the resource contention and learn a cloud application's sensitivity to contention. 
We evaluated variety of machine learning algorithm in terms of prediction accuracy and overhead. Our results show that under moderate level of contention in the cloud, regression and SVR model provide similar accuracy as neural network models. However, NN models will outperform aforementioned models in terms of accuracy in a more contentions environment.
We evaluated the proposed methodology with seventeen benchmarks on a private cloud, Amazon Web Services, and Google Compute Engine. The evaluation results show that the proposed methodology is highly accurate with average errors of only 10.3\%, 3.8\% and 3.4\% for each of the three clouds, respectively. These results demonstrated the feasibility of performance prediction for ordinary cloud users without the need of knowing or controlling the underlying execution environment.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "19-ispass"
%%% End:


==> limits.tex <==
As mentioned in Section~\ref{sec:evaluations}, one of the factors affecting the accuracy of the proposed methodology is that our memory micro-benchmark only profiles contentions for the off-chip memory resources and has a single memory access pattern. To improve accuracy, we will add micro-benchmarks with smaller working sets to profile cache contentions and include micro-benchmarks with other memory access patterns in the future. We will also include micro-benchmarks to profile the contention at network resources so that the proposed methodology can be extended to network-intensive applications.

Additionally, the evaluation results show that the predictive models currently used in the proposed methodology cannot predict unusually-long executions (outliers). We plan to incorporate extreme value theory with Neural Network to improve the prediction accuracy for these unusual cases~\cite{2018-Rudd-TPAMI}. We will also investigate predictive techniques for applications experiencing changes in the contention during execution.

Another limitation of this work is that our benchmarks are using the same inputs during the training and prediction phases. The goal of this research is to investigate the feasibility of predicting cloud application's performance under resource contentions from the ordinary cloud user's perspective. Hence, we intentionally used the same inputs to eliminate the impact from input variations, so that the performance fluctuation is the main cause of resource contentions, and the evaluation can be focused on the proposed methodology's accuracy to predict the impacts of resource contentions. In the future, we will extend the proposed methodology to include predictions under input variations. Nonetheless, it is worth noting that many cloud applications, such as certain web/data serving applications, machine-learning training, and inference applications, may experience few changes in the inputs or inputs sizes for a long period of execution. Therefore, the methodology presented in this paper may already work well for these applications.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "19-ispass"
%%% End:

